How to Approximate A Set Without Knowing Its Size In Advance

The dynamic approximate membership problem asks to represent a set S of size n, whose elements are provided in an on-line fashion, supporting membership queries without false negatives and with a false positive rate at most epsilon. That is, the membership algorithm must be correct on each x in S, and may err with probability at most epsilon on each x not in S. We study a well-motivated, yet insufficiently explored, variant of this problem where the size n of the set is not known in advance. Existing optimal approximate membership data structures require that the size is known in advance, but in many practical scenarios this is not a realistic assumption. Moreover, even if the eventual size n of the set is known in advance, it is desirable to have the smallest possible space usage also when the current number of inserted elements is smaller than n. Our contribution consists of the following results: - We show a super-linear gap between the space complexity when the size is known in advance and the space complexity when the size is not known in advance. - We show that our space lower bound is tight, and can even be matched by a highly efficient data structure.

==> UpperBoundDynamic.tex <==
\section{A Matching Upper Bound for the Dynamic Problem}\label{Sec:UpperBoundDynamic}

\Gil{In progress.}

Lovett and Porat \cite{LovettP10} have recently proved that any dynamic approximate set membership data structure for sets of size $n$ with false positive rate $\epsilon$ must utilize at least $n \log(1/\epsilon) + \Omega(n / \log(1/\epsilon))$ bits, for all sufficiently small $\epsilon$. This is a somewhat surprising result, separating the dynamic setting from the static setting when the false positive rate is a small constant. In this section we show that the lower bound of Lovett and Porat is in fact tight. That is, we construct a dynamic approximate set membership data structure for sets of size $n$ with false positive rate $\epsilon$ that uses $n \log(1/\epsilon) + O(n / \log(1/\epsilon))$ bits.

\paragraph{The construction.} Given $n \in \mathbb{N}$ and $\epsilon > 0$, set $\alpha = \sqrt{2 + \log e / \log(1/\epsilon)}$, $n_1 = (1 - \alpha)n$, $\epsilon_1 = (\epsilon/4)^{1+\alpha}$, $n_2 = n - n_1$, and $\epsilon_2 = \epsilon \cdot e 2^{- \frac{1}{\sqrt{\log(1/\epsilon)}}}$. Let $\mathcal{H}_1$ be a universal collection of functions $h_1 : U \rightarrow [n_1/\epsilon_1]$, and let $\mathcal{H}_2$ be a universal collection of functions $h_2 : U \rightarrow [n_2/\epsilon_2]$.
\begin{enumerate}
\item Allocate a dynamic dictionary $\mathcal{D}_1$ for storing sets of size $n_1$ from the universe $[n_1/\epsilon_1]$, sample $h_1 \leftarrow \mathcal{H}_1$, and store the value $h_1(x)$ for each of the first $n_1$ elements $x_1, \ldots, x_{n_1}$.

\item When the element $x_{n_1 + 1}$ arrives, first compress $\mathcal{D}_1$ as follows: Allocate a static approximate set membership data structure $\mathcal{S}$ for storing $n_1$ elements from the universe $[n_1/\epsilon_1]$ with a false positive rate $\epsilon_{\mathcal{S}} = \epsilon \cdot 2^{- \frac{1}{\log(1/\epsilon)}}$. Enumerate all elements that are stored in $\mathcal{D}_1$, insert them into $\mathcal{S}$, and deallocate the space used by $\mathcal{D}_1$.

    Then, allocate a dynamic dictionary $\mathcal{D}_2$ for storing sets of size $n_2$ from the universe $[n_2/\epsilon_2]$, sample $h_2 \leftarrow \mathcal{H}_2$, and store the value $h_2(x)$ for each of the remaining $n_2$ elements $x_{n_1 + 1}, \ldots, x_n$.

\item The lookup operation for an element $x \in U$ is defined s follows: If at most $n_1$ elements were inserted so far, return the result of a lookup for $h_1(x)$ in $\mathcal{D}_1$. Otherwise (i.e., more than $n_1$ elements were inserted so far), return the logical OR of a lookup for $h_1(x_1)$ in $\mathcal{S}$ and a lookup for $h_2(x)$ in $\mathcal{D}_2$.
\end{enumerate}

\begin{theorem}
For any constant $0 < \epsilon < 1$ and sufficiently large $n$, there exists a dynamic approximate membership data structure for $n$ elements with false positive rate $\epsilon$ that uses space $n \log(1/\epsilon) + O(n / \log(1/\epsilon))$ bits.
\end{theorem}


\Gil{sketch}

Ignoring the efficiency of insertions (i.e., using information-theoretic representations and rebuilding on each insertion), $\mathcal{D}_1$ needs $n_1 \log(1/\epsilon_1) + n_1 \log e$  bits, $\mathcal{S}$ needs $n_1 \log(1/\epsilon_{\mathcal{S}}) + o(n_1)$ bits, and $\mathcal{D}_2$ needs $n_2 \log(1/\epsilon_2) + n_2 \log e$ bits. Therefore the total amount of space that is needed is
\begin{MyEqn}
& & \max \left\{ n_1 \log(1/\epsilon_1) + n_1 \log e, \right. \\
& & \qquad \qquad \left. n_1  \log(1/\epsilon_{\mathcal{S}}) + o(n_1) + n_2 \log(1/\epsilon_2) + n_2 \log e \right\}
\end{MyEqn}
%
We bound each of these terms as follows:

\Gil{Space used by $\mathcal{D}_1$:}

\begin{MyEqn}
& & n_1 \log(1/\epsilon_1) + n_1 \log e \\
& & \quad = (1 - \alpha^2) n \log(4/\epsilon) + (1 - \alpha) n \log e \\
& & \quad = (1 - \alpha^2) n \log(1/\epsilon) + 2 (1 - \alpha^2) n + (1 - \alpha) n \log e \\
& & \quad = (1 - \alpha^2) n \log(1/\epsilon) + (2 + \log e) n \\
& & \quad \leq n \log(1/\epsilon) - \alpha^2 n \log(1/\epsilon) + (2 + \log e) n \\
& & \quad = n \log(1/\epsilon) .
\end{MyEqn}

\Gil{Space used by $\mathcal{S}$ and $\mathcal{D}_2$:}

\begin{MyEqn}
& & n_1  \log(1/\epsilon_{\mathcal{S}}) + o(n_1) + n_2 \log(1/\epsilon_2) + n_2 \log e \\
%& & \quad = n_1  \log(1/\epsilon) + n_1 \log(\epsilon / \epsilon_{\mathcal{S}}) + o(n_1) + n_2 \log(1/\epsilon_2) + n_2 \log e \\
& & \quad = n \log(1/\epsilon) +  n_1 \log(\epsilon / \epsilon_{\mathcal{S}}) + o(n_1) + n_2 \log(\epsilon e / \epsilon_2)  \\
& & \quad = n \log(1/\epsilon) + (1 - \alpha)n \cdot \frac{1}{\log(1/\epsilon)} + o(n_1) + \alpha n \cdot \frac{1}{\sqrt{\log(1/\epsilon)}} \\
& & \quad \leq n \log(1/\epsilon) + n \cdot \frac{1}{\log(1/\epsilon)} + o(n) + \alpha n \cdot \frac{1}{\sqrt{\log(1/\epsilon)}} \\
& & \quad = n \log(1/\epsilon) + \frac{\sqrt{2 + \log e} + 1}{\log(1/\epsilon)} \cdot n + o(n)\\
\end{MyEqn}


\Gil{The false positive rate is $\epsilon_1 + (1 - \epsilon_1) (\epsilon_{\mathcal{S}} + \epsilon_2)$.}




%\Rasmus{In the Porat-Lovett setting with fixed space allocated there is a lower bound on space overhead of $\Omega(n/\log(1/\varepsilon))$ bits. Though not stated in their paper, I think this is in fact near-optimal: Use a dictionary-based scheme that uses $n\log(1/\varepsilon)(1+o(1))+O(n)$ bits to achive FPR $\varepsilon^{1+o(1)}$, and apply it to the first $n'=n-\omega(n/\log(1/\varepsilon))$ insertions. This should use at most $n\log(1/\varepsilon)$ bits. Then use a static approximate membership data structure to ``compress'' the set stored to size $n'\log(1/\varepsilon)$ bits with FPR $\varepsilon - 1/\log^2 n$. Finally, handle the last insertions again using a dictionary and FPR $1/\log^3 n$.} 
